On the computation of the infinity Wasserstein distance and the Wasserstein Projection Problem

Computing the infinity Wasserstein distance and retrieving projections of a probability measure onto a closed subset of probability measures are critical sub-problems in various applied fields. However, the practical applicability of these objects is limited by two factors: either the associated quantities are computationally prohibitive or there is a lack of available algorithms capable of calculating them. In this paper, we propose a novel class of Linear Programming problems and a routine that allows us to compute the infinity Wasserstein distance and to compute a projection of a probability measure over a generic subset of probability measures with respect to any $p$-Wasserstein distance with $p\in[1,\infty]$.

==> math_input.tex <==
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}



\def \sumX{\sum_{x \in X}}
\def \sumY{\sum_{y \in X}}
\def \sumXY{\sum_{(x,y)\in X\times X}}
\def \sumNct{\sum_{(x,y)\in \Nct}}
\def \sumNctc{\sum_{(x,y)\in X \times Y \backslash \Nct }}
\def \sumOct{\sum_{y \in \Oct}}
\def \sumIct{\sum_{x \in \Ict}}
\def \sumFut{\sum_{(x,y) \in \Fut}}
\def \sumEct{\sum_{x \in \Ect}}
\def \sumUct{\sum_{y \in \Uct}}

\def \forallx{\forall x \in X}
\def \forally{\forall y \in X}
\def \forallxy{\forall (x,y) \in X\times Y}
\def \forallNct{\forall (x,y)\in \Nct}
\def \forallFut{\forall (x,y)\in \Fut}

\def \erre{\mathbb{R}}
\def \erred{\erre^d}

\def \ct{c^{(t)}}
\def \cu{c^{[t]}}
\def \ctxy{\ct_{x,y}}
\def \Nct{N_t}
\def \Fut{F^{[t]}_c} 
\def \Oct{B_t(x)}
\def \Ict{B_t(y)}
\def \Uct{U_c^{[t]}(x)}
\def \Ect{E_c^{[t]}(y)}
\def \Tinf{\mathbb{T}_c^{\infty}}
\def \Winf{W^{(\infty)}_c}

\def \NFs{\mathcal{N}^{(t)}_{\mu,\nu}}
\def \FFs{\mathcal{Z}^{[t]}_{\mu,\nu}}
\def \MNFs{\Theta^{(t)}_{\mu,\nu}}

\def \bside{\mathbb{B}^{(t)}_s}
\def \cside{\mathbb{S}^{[t]}_c}
\def \bsidein{\mathbb{B}^{(t)}_\infty}

%%%%%%%%%%% LETTERE %%%%%%%%%%%%%%%%%%%%%

\def \t{\textbf{t}}
\def \x{\textbf{x}}
\def \y{\textbf{y}}
\def \z{\textbf{z}}
\def \A{\textbf{A}}
\def \O{\mathbf{O}}
\def \D{\mathbf{D}}
\def \B{\mathbb{B}}

%%%%%%%%%%%%% INSIEMI %%%%%%%%%%%%%%%%

\def \PP{\mathcal{P}}
\def \II{\mathcal{I}}
\def \CC{\mathcal{C}}
\def \UU{\mathcal{U}}
\def \BB{\mathcal{B}}
\def \FF{\mathcal{F}}
\def \GG{\mathcal{G}}
\def \RR{\mathcal{R}}
\def \AA{\mathcal{A}}
\def \MM{\mathcal{M}}
\def \LL{\mathcal{L}}
\def \NN{\mathcal{N}}

\def \probX{\PP(X)}
\def \PPX{\probX}
\def \probY{\PP(Y)}
\def \PPY{\probY}
\def \PPXy{\PP(X\times Y_1)}
\def \PPxY{\PP(X_2\times Y)}
\def \probzi{\PP(Z_i)}
\def \probrn{\PP(\erren)}
\def \FFmn{\FF(\mu,\nu)}
\def \Pimn{\Pi_{\mu,\nu}}
\def \IImn{\II(\mu,\nu)}

\def \Xfu{X\times Y_1}
\def \Xfd{X_2\times Y}

\def \rpos{[0,\infty)}
\def \erre{\mathbb{R}}
\def \erren{\erre^N}
\def \zet{\mathbb{Z}}

\def \CCu{\CCinf_1}
\def \CCd{\CCinf_2}
\def \CCinf{\CC^{(\infty)}}

%%%%%%%%%%%%% INTEGRALI %%%%%%%%%%%%%%%%%%

\def \intXY{\int_{X\times Y}}
\def \intXZY{\int_{X\times Z \times Y}}
\def \intX{\int_{X}}
\def \intY{\int_{Y}}
\def \intxY{\int_{X_2\times Y}}
\def \intXy{\int_{X\times Y_1}}
\def \intmed{\dfrac{1}{2\pi}\int_{[0,2\pi]}}

\def \intNct{\int_{\Nct}}
\def \intIct{\int_{\Ict}}
\def \intOct{\int_{\Oct}}
\def \intNctc{\int_{\erre^d\times\erre^d\backslash\Nct}}
\def \intEct{\int_{\Ect}}
\def \intFut{\int_{\Fut}}

\def \GBP{G_{X\to Y}}
\def \EBP{E_{X\to Y}}
\def \kgam{\mathcal{K}^{\gamma}}
\def \pila{\pi^{\lambda}}
\def \EMDa{\widehat{EMD}_\alpha}

%%%%%%%%%%%%%%%%% PROIEZIONI %%%%%%%%%%%%%%%

\def \proj#1{(\mathfrak{p}_{#1})_\#}
\def \projX{(\mathfrak{p}_X)_\#}
\def \projY{(\mathfrak{p}_Y)_\#}
\def \projXY{(\mathfrak{p}_{X\times Y})_\#}
\def \projx{(\mathfrak{p}_{X_1})_\#}
\def \projxx{(\mathfrak{p}_{X_2})_\#}
\def \projxxyy{(\mathfrak{p}_{X_2})_\#}
\def \projyyxx{(\mathfrak{p}_{X_2})_\#}
\def \projy{(\mathfrak{p}_{Y_2})_\#}
\def \projyy{(\mathfrak{p}_{Y_1})_\#}
\def \projzi{(\mathfrak{p}_{Z_i})_\#}
\def \projXy{(\mathfrak{p}_{X\times Y_1})_\#}
\def \projxY{(\mathfrak{p}_{X_2\times Y})_\#}
\def \projxy{(\mathfrak{p}_{Y_1\times X_2})_\#}
\def \projyx{(\mathfrak{p}_{X_1\times Y_2})_\#}

\def \pr#1{(\mathfrak{p}_{#1})}
\def \prX{(\mathfrak{p}_{X})}
\def \prY{(\mathfrak{p}_{Y})}
\def \prXy{(\mathfrak{p}_{X\times Y_1})}
\def \prxY{(\mathfrak{p}_{X_2\times Y})}
\def \prxy{(\mathfrak{p}_{X_2\times Y_1})}
\def \thpr{\pr_{\theta}}
\def \thprth{\pr_{\theta^{\perp}}}
%%%%%%%%%%%%% INFIMUM %%%%%%%%%%%%%%%%%%%%

\def \infpi{\inf_{\pi \in \Pimn}}
\def \minpi{\min_{\pi \in \Pimn}}
\def \infcf{\inf_{\ff \in \FFmn}}
\def \infcfn{\inf_{\FFN \in \FFmn}}
\def \infIp{\inf_{\sigma \in \II(\mu,\nu)}}
\def \minff{\min_{\ff \in \FFmn}}
\def \maxNFs{\max_{\eta\in\NFs}}


\def \mn{(\mu,\nu)}
\def \ff{(\funo,\fdue)}
\def \FFN{(f^{(1)},\dots,f^{(N)})}
\def \funo{f^{(1)}}
\def \fdue{f^{(2)}}

\def \sigu{\sigma_{|x_2}^{(1)}}
\def \sigd{\sigma_{|y_1}^{(2)}}


%%%% SOMMATORIE %%%%%%

\def \sumX{\sum_{x \in X}}
\def \sumY{\sum_{y \in X}}
\def \sumXY{\sum_{(x,y)\in X\times X}}
\def \sumNct{\sum_{(x,y)\in \Nct}}
\def \sumNctc{\sum_{(x,y)\in (X \times Y) \backslash \Nct }}
\def \sumOct{\sum_{y \in \Oct}}
\def \sumIct{\sum_{x \in \Ict}}
\def \sumFut{\sum_{(x,y) \in \Fut}}
\def \sumEct{\sum_{x \in \Ect}}
\def \sumUct{\sum_{y \in \Uct}}
\def \sumGO{ \sum_{(a_1,a_2) \in G, b_1 \in O^{(1)}_{t_1}(a_1)}}
\def \sumGI{ \sum_{(b_1,b_2)\in G, a_2\in I^{(2)}_{t_2}(b_2)}}

%%%%%% FOR ALLS %%%%%%%%%%

\def \forallx{\forall x \in X}
\def \forally{\forall y \in X}
\def \forallxy{\forall (x,y) \in X\times X}
\def \forallNct{\forall (x,y)\in \Nct}
\def \forallFut{\forall (x,y)\in \Fut}

%%%%%%% COST FUNCTIONS %%%%%%%

\def \ct{c^{(t)}}
\def \cu{c^{[t]}}
\def \ctxy{\ct_{x,y}}
\def \cinfu{c^{(\infty)}_1}
\def \cinfd{c^{(\infty)}_2}

%%%%%%%%%% INSIEMI TRONCATE %%%%%%%%%%%%%%

\def \Nct{N_t}
\def \Fut{F^{[t]}_c} 
\def \Oct{B_t(x)}
\def \Ict{B_t(y)}
\def \Uct{U_c^{[t]}(x)}
\def \Ect{E_c^{[t]}(y)}

%%%%%%%%% FUNZIONALI %%%%%%%%%%%%%

\def \Tinf{\mathbb{T}_c^{\infty}}
\def \Winf{W^{(\infty)}_c}
\def \NFs{\mathcal{N}^{(t)}_{\mu,\nu}}
%\def \FFs{\mathcal{Z}^{[t]}(\mu,\nu)}
\def \FFseta{\mathcal{Z}^{[t,\eta^*]}_{\mu,\nu}}
\def \MNFs{\Theta^{(t)}_{\mu,\nu}}
\def \bside{\mathbb{B}^{(t)}_s}
\def \cside{\mathbb{S}^{[t]}_c}
\def \bsidein{\mathbb{B}^{(t)}_\infty}
\def \T{\mathbb{T}_c}
\def \TC{\mathbb{TC}}
\def \ST{\mathbb{CT}_c}
\def \Z{\mathbb{Z}}

\def \a{\textbf{a}}
\def \b{\textbf{b}}

\def \erreinf{\erre\cup\{+\infty\}}
\def \Leb{\mathcal{L}}
\def \enne{\mathbb{N}}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

==> tables/tabProjWinfThresholds.tex <==
\begin{table}[t]
\centering
\begin{tabular}{cccc}
\toprule
$\theta$ & $32 \times 32$ & $64 \times 64$ & $128 \times 128$ \\
\midrule 
\csvreader[
late after line=\\,
]
{tables/tabProjWinftyThresholds.csv}{1=\barr, 2=\avgi, 3=\maxi, 4=\avgii, 5=\maxii, 6=\avgiii, 7=\maxiii}
{\numDi{\barr} & \numD{\avgi} (\numD{\maxi}) & \numD{\avgii} (\numD{\maxii}) & \numD{\avgiii} (\numD{\maxiii})}
\bottomrule
\end{tabular}
\caption{Mean threshold values $\bar{t}$ reached by the Climbing Algorithm in the computation of the $W_{\infty}$-projection. Maximum values are provided in parentheses.}
\label{tab:ClaProjWinftyThresholds}
\end{table}


% \begin{table}[t]
% \centering
% \pgfplotstableread[col sep=comma]{tables/tabProjWinftyThresholds.csv}\loadedtable
% \pgfplotstabletypeset[
% columns={tau, Cla 32 mean, Cla 32 max},
% columns/tau/.style={precision=3, column name=$\theta$,
% zerofill},
% columns/Cla 32 mean/.style={column name=$32 \times 32$},
% every head row/.style={before row={\toprule}, after row=\midrule},
% every last row/.style={after row=\bottomrule},
% ]\loadedtable
% \caption{Mean threshold values $\bar{t}$ reached by the Climbing Algorithm in the computation of the $W_{\infty}$-projection. Maximum values are provided in parentheses.}
% \label{tab:ClaProjWinftyThresholds}
% \end{table}

